Spatial Self-Interference Isolation for In-Band Full-Duplex Wireless: A Degrees-of-Freedom Analysis

The challenge to in-band full-duplex wireless communication is managing self-interference. Many designs have employed spatial isolation mechanisms, such as shielding or multi-antenna beamforming, to isolate the self-interference wave from the receiver. Such spatial isolation methods are effective, but by confining the transmit and receive signals to a subset of the available space, the full spatial resources of the channel be under-utilized, expending a cost that may nullify the net benefit of operating in full-duplex mode. In this paper we leverage an antenna-theory-based channel model to analyze the spatial degrees of freedom available to a full-duplex capable base station, and observe that whether or not spatial isolation out-performs time-division (i.e. half-duplex) depends heavily on the geometric distribution of scatterers. Unless the angular spread of the objects that scatter to the intended users is overlapped by the spread of objects that backscatter to the base station, then spatial isolation outperforms time division, otherwise time division may be optimal.

==> DocGraphics/FD_BS_Clusters_old.tex <==
\tikzstyle{block} = [draw,fill=KeynoteBlue!30,minimum size=2em]
\tikzstyle{bigBlock} = [draw,fill=KeynoteRed!50,minimum size=1.5em]
\tikzstyle{scatterer} = [draw,fill=gray!50,minimum size=2em]
\tikz[auto, decoration={
  markings,
  mark=at position 1.0 with {\arrow{>}}}
]{
\coordinate (T1) at (-3,0);
\coordinate (R1) at (-1,4);
\coordinate (T2) at (1,4);
\coordinate (R2) at (3,0);
%
\node [circle,draw,KeynoteBlue] (S11) at (-1.2,1.3) [minimum size=60pt] {};
\node [circle,draw,KeynoteRed] (S12) at (0.2,2.1) [minimum size=60pt] {};
\node [circle,draw,KeynoteGreen] (S22) at (1,1.2) [minimum size=60pt] {};
%
\draw[KeynoteBlue] (T1) -- (tangent cs:node=S11,point={(T1)},solution=1);
\draw[KeynoteBlue] (T1) -- (tangent cs:node=S11,point={(T1)},solution=2);
%
\draw[KeynoteBlue] (R1) -- (tangent cs:node=S11,point={(R1)},solution=1);
\draw[KeynoteBlue] (R1) -- (tangent cs:node=S11,point={(R1)},solution=2);
%
%
\draw[KeynoteRed] (T2) -- (tangent cs:node=S12,point={(T2)},solution=1);
\draw[KeynoteRed] (T2) -- (tangent cs:node=S12,point={(T2)},solution=2);
%
\draw[KeynoteRed] (R1) -- (tangent cs:node=S12,point={(R1)},solution=1);
\draw[KeynoteRed] (R1) -- (tangent cs:node=S12,point={(R1)},solution=2);
%
\draw[KeynoteGreen] (T2) -- (tangent cs:node=S22,point={(T2)},solution=1);
\draw[KeynoteGreen] (T2) -- (tangent cs:node=S22,point={(T2)},solution=2);
%
\draw[KeynoteGreen] (R2) -- (tangent cs:node=S22,point={(R2)},solution=1);
\draw[KeynoteGreen] (R2) -- (tangent cs:node=S22,point={(R2)},solution=2);
%
%
\node[KeynoteBlue] at ($(S11.center)!40pt!(T1)$) {$\ElevT{11}$};
\node[KeynoteBlue] at ($(S11.center)!38pt!(R1)$) {$\ElevR{11}$};
%
\node[KeynoteRed] at ($(S12.center)!40pt!(T2)$) {$\ElevT{12}$};
\node[KeynoteRed] at ($(S12.center)!40pt!(R1)$) {$\ElevR{12}$};
\node[KeynoteGreen] at ($(S22.center)!38pt!(T2)$) {$\ElevT{22}$};
\node[KeynoteGreen] at ($(S22.center)!40pt!(R2)$) {$\ElevR{22}$};
%
\path (T1)+(-0.25,-0.25) node {$T_1$}
(T2)+(0,+0.25) node {$T_2$}
(R1)+(0,+0.25) node {$R_1$}
(R2)+(+0.25,-0.25) node {$R_2$};
%
\node at ($(R1)!0.5!(T2)+(0,0.75)$) {\underline{FD Base Station}};
\node at ($(T1)+(0,-0.75)$) {{User 1 (Uplink)}};
\node at ($(R2)+(0,-0.75)$) {{User 2 (Downlink)}};
%
\iftoggle{ZChanModel}{}{
\node [circle,draw,KeynoteYellow] (S21) at (-0.2,1) [minimum size=50pt] {};
%
\node[KeynoteYellow] at ($(S21.center)!40pt!(T1)$) {$\ElevT{21}$};
\node[KeynoteYellow] at ($(S21.center)!40pt!(R2)$) {$\ElevR{21}$};
%
\draw[KeynoteYellow] (T1) -- (tangent cs:node=S21,point={(T1)},solution=1);
\draw[KeynoteYellow] (T1) -- (tangent cs:node=S21,point={(T1)},solution=2);
%
\draw[KeynoteYellow] (R2) -- (tangent cs:node=S21,point={(R2)},solution=1);
\draw[KeynoteYellow] (R2) -- (tangent cs:node=S21,point={(R2)},solution=2);
%
}
}
 

==> DocGraphics/FD_BS_fig.tex <==
\tikzstyle{block} = [draw,fill=KeynoteBlue!30,minimum size=2em]
\tikzstyle{bigBlock} = [draw,fill=KeynoteRed!50,minimum size=1.5em]
\tikzstyle{scatterer} = [draw,fill=gray!50,minimum size=2em]
\tikz[auto, decoration={
  markings,
  mark=at position 1.0 with {\arrow{>}}}
]{
\path (0,0)  node (ArrayOneTx)  [ellipse,draw, minimum height = 5em, minimum width = 3em, rotate=-30, fill=KeynoteBlue, nearly transparent]  {$$} 
+(0,-1.2) node {{User 1 (Uplink)}}
+(0,-.4) node {$\bullet\vect{p}_1$}
(ArrayOneTx.center)+(-1,0) node {$\ArrayOneTx$}
;
\path (4.5,4) node (ArrayTwoTx) [ellipse,draw, minimum height = 5em, minimum width = 6em, fill=KeynoteRed, nearly transparent]  {$$}
+(-1,1.3) node {\underline{FD Base Station Rx/Tx Arrays}} 
(ArrayTwoTx.east)+(.3,.2) node {$\ArrayTwoTx$}
(ArrayTwoTx.center)+(-.4,+.3) node{$\bullet\vect{p}_2$}
;
%
%
\path (2.5,4)  node (ArrayOneRx)  [ellipse,draw, minimum height = 5em, minimum width = 6em, rotate=60, fill=KeynoteBlue, nearly transparent]  {$$}
 +(-.4,+.4) node {$\bullet\vect{q}_1$}
(ArrayOneRx.center)+(-1.2,0) node {$\ArrayOneRx$}
;
\path (7,-0) node (ArrayTwoRx) [ellipse,draw, minimum height = 3em, minimum width = 5em, fill=KeynoteRed, nearly transparent]  {$$} 
+(0,-0.8) node {{User 2 (Downlink)}}
(ArrayTwoRx.east)+(.4,0) node {$\ArrayTwoRx$}
(ArrayTwoRx.center)+(-.55,0) node{$\bullet\vect{q}_2$}
;
%
%
%
\path(3.5,2.0) node(S0) [scatterer, minimum size=1.5em] {}
+(-1.35,-.7) node(S1) [scatterer, minimum size=1.5em, rotate=-30] {}
+(3,-0.5)  node(S2) [scatterer, minimum size=1.5em, rotate=20] {}
+(2.5,+0.5)  node(S3) [scatterer, minimum size=1.5em, rotate=-20] {}
+(1.5,-0.35)  node(S4) [scatterer, minimum size=1.5em, rotate=-15] {}
+(-2,0.1)  node(S5) [scatterer, minimum size=1.5em, rotate=-15] {}
+(-3.5,0) node (ScatLabel) {{Scatterers}}
;
\draw[] (ScatLabel) -- (S5);
\draw[] (ScatLabel) -- (S1);
%
\draw[->] (ArrayOneTx.center) -- (xyz cs:x=.5); 
\draw[->] (ArrayOneTx.center) -- (xyz cs:y=.5);
\draw[->] (ArrayOneTx.center) -- (xyz cs:z=.5);
\draw[->,densely dashed] (ArrayOneTx.center) to [above] node {$\vect{k}_1$} (S1);
%
\draw[->] (ArrayOneRx.center) -- +(xyz cs:x=.5); 
\draw[->] (ArrayOneRx.center) -- +(xyz cs:y=.5);
\draw[->] (ArrayOneRx.center) -- +(xyz cs:z=.5);
\draw[->,densely dashed] (ArrayOneRx.center) to [left] node  {$\vect{\kappa}_1$} (S1);
%%
\draw[->] (ArrayTwoTx.center) -- +(xyz cs:x=.5); 
\draw[->] (ArrayTwoTx.center) -- +(xyz cs:y=.5);
\draw[->] (ArrayTwoTx.center) -- +(xyz cs:z=.5);
\draw[->,densely dashed] (ArrayTwoTx.center) to [right] node {$\vect{k}_2$} (S4);
%
\draw[->] (ArrayTwoRx.center) -- +(xyz cs:x=.5); 
\draw[->] (ArrayTwoRx.center) -- +(xyz cs:y=.5);
\draw[->] (ArrayTwoRx.center) -- +(xyz cs:z=.5);
\draw[->,densely dashed] (ArrayTwoRx.center) to node [above] {$\vect{\kappa}_2$} (S4);
%
%
}
%controls (0,1) and (1,0) 

==> DocGraphics/GenieModel.tex <==
\tikzstyle{block} = [draw,fill=KeynoteBlue!30,minimum size=2em]
\tikzstyle{bigBlock} = [draw,fill=KeynoteRed!50,minimum size=1.5em]
\tikzstyle{scatterer} = [draw,fill=gray!50,minimum size=2em]
\tikz[auto, decoration={
  markings,
  mark=at position 1.0 with {\arrow{>}}}
]{
%
\path (0,1) node (T1) {$\stackrel[\infty]{}{T_1}$};
%
\path (0,-1) node (T2) {$\stackrel[\SizeTwoTxPrime]{}{T_2}$};
%
\path (6,1) node (R1) {$\stackrel[\SizeOneRxPrime]{}{R_1}$};
%
\path (6,-1) node (R2) {$\stackrel[\infty]{}{R_2}$};
%
\path 
%(3,0) node  [circle ,draw, minimum size = 4em] (S11) {}
%(2.5,0.5) node  [circle ,draw, minimum size = 2.5em] (S12) {}
(3,0) node  [circle ,draw, minimum size = 4em] (S21) {}
%(3,0) node  [circle ,draw, minimum size = 4em] (S22) {}
;  
%%
\draw (T2.east) to node {} (S21.north west) {}
(T2.east) to node {} (S21.south) {};
\path (S21.west)+(-.5,-.45) node {$\Omega_{2}^{(t)}$};
\draw (R1.west) to node {} (S21.north) {}
(R1.west) to node {} (S21.south east) {};
\path (S21.east)+(.5,.45) node {$\Omega_{1}^{(r)}$};
%
\draw (T1.east) to node {} (S21.north) {}
(T1.east) to node {} (S21.south west) {};
%\path (S21.west)+(.5,.45) node {$\Omega_{2}^{(t)}$};
\draw (R2.west) to node {} (S21.north east) {}
(R2.west) to node {} (S21.south) {};
%
%\draw (T1.east) to node {} (S12.north) {}
%(T1.east) to node {} (S12.south west) {};
%%\path (S21.west)+(.5,.45) node {$\Omega_{2}^{(t)}$};
%\draw (R2.west) to node {} (S12.north east) {}
%(R2.west) to node {} (S12.south) {};
%\path (S21.east)+(.5,.45) node {$\Omega_{1}^{(r)}$};
%%
}


==> DocGraphics/ZChanClustersColored.tex <==
\tikzstyle{block} = [draw,fill=KeynoteBlue!30,minimum size=2em]
\tikzstyle{bigBlock} = [draw,fill=KeynoteRed!50,minimum size=1.5em]
\tikzstyle{scatterer} = [draw,fill=gray!50,minimum size=2em]
\tikz[auto, decoration={
  markings,
  mark=at position 1.0 with {\arrow{>}}}
]{
\coordinate (T1) at (-3,1);
\coordinate (R1) at (3,1);
\coordinate (T2) at (-3,-1);
\coordinate (R2) at (3,-1);
%
\node [circle,draw,KeynoteBlue] (S11) at (0,1) [minimum size=50pt] {};
%\node [circle,draw,KeynoteYellow] (S21) at (-.5,.5) [minimum size=30pt] {};
\node [circle,draw,KeynoteRed] (S12) at (+.5,0) [minimum size=50pt] {};
\node [circle,draw,KeynoteGreen] (S22) at (.5,-0.8) [minimum size=50pt] {};
%
\draw[KeynoteBlue] (T1) -- (tangent cs:node=S11,point={(T1)},solution=1);
\draw[KeynoteBlue] (T1) -- (tangent cs:node=S11,point={(T1)},solution=2);
%
\draw[KeynoteBlue] (R1) -- (tangent cs:node=S11,point={(R1)},solution=1);
\draw[KeynoteBlue] (R1) -- (tangent cs:node=S11,point={(R1)},solution=2);
%%
%\draw[KeynoteYellow] (T1) -- (tangent cs:node=S21,point={(T1)},solution=1);
%\draw[KeynoteYellow] (T1) -- (tangent cs:node=S21,point={(T1)},solution=2);
%%
%\draw[KeynoteYellow] (R2) -- (tangent cs:node=S21,point={(R2)},solution=1);
%\draw[KeynoteYellow] (R2) -- (tangent cs:node=S21,point={(R2)},solution=2);
%
%
\draw[KeynoteRed] (T2) -- (tangent cs:node=S12,point={(T2)},solution=1);
\draw[KeynoteRed] (T2) -- (tangent cs:node=S12,point={(T2)},solution=2);
%
\draw[KeynoteRed] (R1) -- (tangent cs:node=S12,point={(R1)},solution=1);
\draw[KeynoteRed] (R1) -- (tangent cs:node=S12,point={(R1)},solution=2);
%
\draw[KeynoteGreen] (T2) -- (tangent cs:node=S22,point={(T2)},solution=1);
\draw[KeynoteGreen] (T2) -- (tangent cs:node=S22,point={(T2)},solution=2);
%
\draw[KeynoteGreen] (R2) -- (tangent cs:node=S22,point={(R2)},solution=1);
\draw[KeynoteGreen] (R2) -- (tangent cs:node=S22,point={(R2)},solution=2);
%
%
\node[KeynoteBlue] at ($(S11.center)!40pt!(T1)$) {$\ClusterT{11}$};
\node[KeynoteBlue] at ($(S11.center)!40pt!(R1)$) {$\ClusterR{11}$};
%\node[KeynoteYellow] at ($(S21.center)!40pt!(T1)$) {$\ClusterT{21}$};
%\node[KeynoteYellow] at ($(S21.center)!40pt!(R2)$) {$\ClusterR{21}$};
\node[KeynoteRed] at ($(S12.center)!40pt!(T2)$) {$\ClusterT{12}$};
\node[KeynoteRed] at ($(S12.center)!40pt!(R1)$) {$\ClusterR{12}$};
\node[KeynoteGreen] at ($(S22.center)!40pt!(T2)$) {$\ClusterT{22}$};
\node[KeynoteGreen] at ($(S22.center)!40pt!(R2)$) {$\ClusterR{22}$};
%
\path (T1)+(-0.25,0) node {$T_1$}
(T2)+(-0.25,0) node {$T_2$}
(R1)+(+0.25,0) node {$R_1$}
(R2)+(+0.25,0) node {$R_2$};
}
 

==> DocGraphics/ZChanUnipolAchieve.tex <==
\begin{thm}
\label{thm:ZChanOne}
For the spatial $Z$-channel with unipolarized linear arrays, the degree-of-freedom pair $(d_1',d_2')$ is achievable, where 
\begin{align}
d_1' =&\min\left\{2\LenOneTx |\IntT{11}|, 2\LenOneRx |\IntR{11}|\right\} \\
d_2' =& \min\left\{d_{T_2},2\LenTwoRx |\IntR{22}|\right\} 1(\LenOneTx |\IntT{11}| \geq \LenOneRx |\IntR{11}|) \nonumber \\ 
 &+ \min\left\{\delta_{T_2},2\LenTwoRx |\IntR{22}|\right\} 1(\LenOneTx |\IntT{11}| < \LenOneRx |\IntR{11}|),
\end{align}
where $d_{T_2}$ and $\delta_{T_2}$ are given in (\ref{eq:dT2}-\ref{eq:deltaT2}) at the top of the following page. 


\begin{figure*}[!t]
% ensure that we have normalsize text
\normalsize
% Store the current equation number.
\setcounter{MYtempeqncnt}{\value{equation}}
% Set the equation number to one less than the one
% desired for the first equation here.
% The value here will have to changed if equations
% are added or removed prior to the place these
% equations are referenced in the main text.
\setcounter{equation}{22}
\hrulefill
\begin{align}
%
d_{T_2} =& 2 \LenTwoTx |\IntT{22} \setminus \IntT{12}|
+ 2\min \left\{ \vphantom{\left(|\IntT{12}|\right)^+}  \LenTwoTx |\IntT{22} \cap \IntT{12}|,  
(\LenTwoTx |\IntT{12}| - \LenOneRx |\IntR{12}| )^+  +   \LenOneRx |\IntR{12} \setminus \IntR{11}| \right\}^+ \label{eq:dT2}\\
%
%d_{R_2} =& \LenTwoRx |\IntR{22} \setminus \IntR{12}| + \min \left\{ {\scriptstyle \vphantom{\left(|\IntT{12}|\right)^+} \LenTwoRx |\IntR{22} \cap \IntR{12}|,
%\LenTwoRx |\IntR{21}| - \left[\LenOneRx|\IntR{11}| - \left(\LenOneTx \IntT{11} \setminus \IntT{21} + (\LenOneTx |\IntT{21}| - \LenTwoRx |\IntR{21}|)^+ \right) \right]^+ } \right\} \label{eq:d2r}\\
%
\delta_{T_2} =& 2\LenTwoRx |\IntT{22} \setminus \IntT{12}| + 2\min \left\{ {\scriptstyle\vphantom{\left(|\IntR{12}|\right)^+} \LenTwoRx |\IntT{22} \cap \IntT{12}|,
\LenTwoRx |\IntT{12}| - \left[\LenOneRx|\IntT{11}| - \left(\LenOneTx \IntR{11} \setminus \IntR{12} + (\LenTwoTx |\IntR{12}| - \LenOneRx |\IntT{12}|)^+ \right) \right]^+ } \right\} \label{eq:deltaT2}
%
%\\ \delta_{R_2} =& \LenTwoRx |\IntR{22} \setminus \IntR{21}| + \min\left\{\LenTwoRx|\IntR{22} \cap \IntR{21}|,
%(\LenTwoRx|\IntR{21}| - \LenOneTx|\IntT{21}|)^+ + \LenOneTx|\IntT{21} \setminus \IntT{11}| \right\}^+\label{eq:delta2r}
\end{align}
%
%\begin{align}
%%d_{T_1} =&  \LenOneTx |\IntT{11} \setminus \IntT{21}|
%%+ \min \left\{ \vphantom{\left(|\IntT{12}|\right)^+}  \LenOneTx |\IntT{11} \cap \IntT{21}|,  
%%\max (\LenOneTx |\IntT{21}|, \LenTwoRx |\IntR{21}| ) -  \LenTwoRx |\IntR{22} \cap \IntR{21}| \right\}^+ \label{eq:d1t}\\
%%
%d_{R_1} =& 2\LenOneRx |\IntR{11} \setminus \IntR{12}| + 2\min \left\{ {\scriptstyle \vphantom{\left(|\IntT{12}|\right)^+} \LenOneRx |\IntR{11} \cap \IntR{12}|, 
%%\right. \nonumber \\  & \left. \hspace{200pt} 
%\LenOneRx |\IntR{12}| - \left[\LenTwoRx|\IntR{22}| - \left(\LenTwoTx \IntT{22} \setminus \IntT{12} + (\LenTwoTx |\IntT{12}| - \LenOneRx |\IntR{12}|)^+ \right) \right]^+} \right\}\\
%%
%%\delta_{T_1} =& \LenOneRx |\IntT{11} \setminus \IntT{21}| + \min \left\{ {\scriptstyle \vphantom{\left(|\IntR{21}|\right)^+} \LenOneRx |\IntT{11} \cap \IntT{21}|,
%%% \right. \nonumber \\  & \left. \hspace{200pt} 
%%\LenOneRx |\IntT{21}| - \left[\LenTwoRx|\IntT{22}| - \left(\LenTwoTx \IntR{22} \setminus \IntR{21} + (\LenOneTx |\IntR{21}| - \LenTwoRx |\IntT{21}|)^+ \right) \right]^+ } \right\} \\
%%
%\delta_{R_1} =& 2\LenOneRx |\IntR{11} \setminus \IntR{12}| + 2\min\left\{\LenOneRx|\IntR{11} \cap \IntR{12}|,
%\max(\LenOneRx|\IntR{12}|, \LenTwoTx|\IntT{12}|)- \LenTwoTx|\IntT{22}\cap \IntT{12}|\right\}^+\label{eq:delta1r}
%\end{align}
% Restore the current equation number.
\setcounter{equation}{\value{MYtempeqncnt}}
% IEEE uses as a separator
\hrulefill
% The spacer can be tweaked to stop underfull vboxes.
\vspace*{4pt}
\end{figure*}
%
\end{thm}
\setcounter{equation}{24}

%\begin{align}
%\label{eq:dT2DOF}
%&d_{T_2} =  2\LenTwoTx |\IntT{22} \setminus \IntT{12}| \\
%&+2\min \left\{\!\!\!\!
%\begin{tabular}{c}
%$\LenTwoTx |\IntT{22} \cap \IntT{12}|$, \tabularnewline 
%$(\LenTwoTx |\IntT{12}| - \LenOneRx |\IntR{12}| )^+  +   \LenOneRx |\IntR{12} \setminus \IntR{11}|$
%\end{tabular} 
% \!\!\!\! \right\}, \nonumber
%\end{align}

\begin{IEEEproof}
We prove case where $\LenOneTx |\IntT{11}| \geq \LenOneRx |\IntR{11}|$. In this case we must show achievability of the degree of freedom pair
\begin{align}
d_1' &=2\LenOneRx |\IntR{11}|, \label{eq:d1PrimeCase1} \\
d_2' &=\min\left\{d_{T_2},2\LenTwoRx |\IntR{22}|\right\}, \label{eq:d2PrimeCase1}
\end{align}
where
\begin{align}
&d_{T_2} =  2\LenTwoTx |\IntT{22} \setminus \IntT{12}| + \nonumber \\
& \min \left\{ \!\!\!
\begin{tabular}{c}
$2\LenTwoTx |\IntT{22} \cap \IntT{12}|$, \tabularnewline 
$2(\LenTwoTx |\IntT{12}| - \LenOneRx |\IntR{12}| )^+  +   2\LenOneRx |\IntR{12} \setminus \IntR{11}|$
\end{tabular} 
\!\!\! \right\}. \label{eq:T2DOF}
\end{align}
The proof in the $\LenOneTx |\IntT{11}| < \LenOneRx |\IntR{11}|$ is analogous. 
%
\subsubsection{Formalizing the Channel Model}
To ease the analysis, we cast the channel model of (\ref{eq:Zchan1}-\ref{eq:Zchan2}) into the notation of linear operators on Hilbert spaces. 
Let $\TxSpace{j}$ be the space of all field distributions that transmitter $T_j$'s array of length $\LenTx$ can radiate towards the available scattering clusters, $\IntT{jj}\cup\IntT{ij}$ (both signal-of-interest and interference). In the vernacular of \cite{TsePoon05DOF_EM}, $\TxSpace{j}$ is the space of field distributions array-limited to $\LenTx$ and wavevector-limited to $\IntT{jj}\cup\IntT{ij}$.
To be precise, define $\TxSpace{j}$ to be the Hilbert space of all square-integrable functions  $X_j:\IntT{jj}\cup\IntT{ij}\rightarrow \mathbb{C}$, that can be expressed as
$$
X_j(t) = \int_{-\LenTx}^{\LenTx} \responseTx(t,p) x_j(p)\, dp,\ \quad t\in \IntT{jj}\cup\IntT{ij}
$$
for some $x_j(p),\ p\in [-\LenTx,\LenTx]$. The inner product between two member functions, $U_j,V_j\in\TxSpace{j}$, is the usual inner product
$$
\langle U_j,V_j\rangle = \int_{\IntT{jj}\cup\IntT{ij}} U_j(t)V_j^*(t)\, dt.
$$
Likewise let $\RxSpace{i}$ be the space of field distributions that can be incident on receiver $R_i$ from the available scattering clusters, $\IntR{ii}\cup\IntR{ij}$, and resolved by an array of length $\LenRx$.
More precisely, $\RxSpace{i}$ is the Hilbert space of all square-integrable functions  $Y_i:\IntR{ii}\cup\IntR{ij} \rightarrow \mathbb{C}$, that can be expressed as  
$$
Y_i(\tau) = \int_{-\LenRx}^{\LenRx} \responseRx^*(q,\tau) y_i(q)\, dq,\ \quad \tau\in \IntR{ii}\cup\IntR{ij}
$$
for some $y_i(q),\ q\in [-\LenRx,\LenRx]$, with the usual inner product. 
From \cite{TsePoon05DOF_EM}, we know that the dimension of these array-limited and wavevector-limited transmit and receive spaces are, respectively, 
\begin{align}
\dim \TxSpace{j} &= 2\LenTx |\IntT{jj}\cup\IntT{ij}|\text{, and} \\
\dim \RxSpace{i} &= 2\LenRx |\IntR{ii}\cup\IntR{ij}|.
\end{align}
%
We can think of the scattering integrals in (\ref{eq:Zchan1}-\ref{eq:Zchan2}) as operators mapping from one Hilbert space to another. Define the operator $\ScatOp{ij}:\TxSpace{j}\rightarrow\RxSpace{i}$ by
%\begin{equation}
%(\ScatOp{ij}X_j)(\tau) = \int_{\IntT{ij}} \Scat{ij}(\tau,t) X_j(t)\,dt, \qquad \tau \in \IntR{ij}
%\end{equation}
%\evanNote{Probably should be $\tau \in \IntR{ij}\cup \IntR{ii}$ to be more precise, only nonzero in $\IntR{ij}$.}
\begin{equation}
(\ScatOp{ij}X_j)(\tau) = \int_{\IntT{ij} \cup \IntT{jj}} \!\!\!\!\!\!\!\!\! \Scat{ij}(\tau,t) X_j(t)\,dt,\  \tau \in \IntR{ij}\cup \IntR{ii}.
\end{equation}
%
We can now write the channel model (\ref{eq:Zchan1}-\ref{eq:Zchan2}) in operator notation as 
\begin{align}
Y_1 &= \ScatOp{11}X_1 + \ScatOp{12}X_2 + Z_2\\
Y_2 &= \ScatOp{22}X_2 + Z_2,
\end{align}
where $X_j \in \RxSpace{j}$, for $j=1,2$ and $Y_i, Z_i \in \RxSpace{i}$ for $i=1,2$.
%where $X_1 \in \TxSpace{1}$, $X_2 \in \TxSpace{2}$, $Y_1, Z_1 \in \RxSpace{1}$, and $Y_2, Z_2 \in \RxSpace{2}$.
%
We now begin the achievability steps.



\input{AchieveSteps_v2}
%\newpage
\input{AchieveSteps_v1}


\end{IEEEproof}





==> RelatedWork.tex <==


\subsection{Degrees of Freedom of the MIMO Interference Channel}

In \cite{Jafar07MIMOInterferenceDoF}, the degrees of freedom (DoF) of the two-user vector interference channel is analyzed.  The authors consider a two-user interference channel where users 1 and 2 have $M_1$ and $M_2$, transmit antennas and $N_1$ and $N_2$ receive antennas. The channel matrices are assumed to be full rank. 
The DoF is defined as 
\begin{equation}
\eta({\rm INT}) = \lim_{{\sf snr} \rightarrow \infty} \frac{C_\Sigma({\sf snr})}{\log({\sf snr})},
\end{equation}
where $C_\Sigma({\sf snr})$ is the maximum achievable sum rate. 
Assuming, without loss of generality, that $\max(M_1,N_1) > \max(M_2,N_2)$, the authors show
\begin{align}
\eta_{\rm INT} &= \min(M_1,N_1) \nonumber \\
& \qquad + \min(M_2 - N_1, N_2)^+ 1(M_1 > N_1)\nonumber \\
& \qquad + \min(M_2, N_2-M_1)^+ 1(M_1 < N_1) \nonumber \\
& = \min\{{\scriptstyle M_1 + M_2, N_1 + N_2, \max(M_1,N_2), \max(M_2,N_1)}\}
\label{eq:MIMODoF}.
\end{align}

The first term in eq. \ref{eq:MIMODoF} is the interference-free point-to-point DoF of user 1, and the second term is the DoF left over to user 2 if it avoids generating interference at $R_1$. The achievability is based on an SVD of the interference channel matrices. The SVD of each of the channel responses,  with respect to the interference matrices, converts each of the MIMO channels a into a set of parallel interference channels, where each Eigen input corresponding to a non-zero singular value is an input that causes interference at the other receiver, and the each Eigen input corresponding to a zero singular value is an interference free input. 
%To show achievability of eq. \ref{eq:MIMODoF}, ...

This vector interference channel is basically the discretized version of the continuous array problem we seek to solve, where the scattering is assumed to be rich enough for all channel matrices to be full-rank. We should able to recover eq. \ref{eq:MIMODoF} via a uniform sampling of the continuous arrays, when the environment is fully scattered.  

\subsection{EM Approach to Degrees of Freedom}

In \cite{TsePoon05DOF_EM} the spatial degrees of freedom of a P2P wireless channel with continuous arrays. Transmit and receiver spherical arrays of aperture sizes $\mathcal{A}^{(t)}$ and $\mathcal{A}^{(r)}$ are considered, and the scattering is assumed clustered over angular intervals $\Omega^{(t)}$ and $\Omega^{(r)}$ with respect to the transmitter and receiver respectively. The degrees of freedom for this channel are shown to be

\begin{equation}
{\sf DOF_{P2P}} = \min\{\mathcal{A}^{(t)}|\Omega^{(t)}|,\mathcal{A}^{(r)}|\Omega^{(r)}|\}.
\end{equation}

In the case of a fully scattered environment $|\Omega^{(t)}| =  |\Omega^{(r)}| = 4\pi$ steradians, thus
\begin{equation}
{\sf DOF_{P2P}} = 4\pi\min\{\mathcal{A}^{(t)},\mathcal{A}^{(r)}\}.
\end{equation}


==> converseProof_sketch.tex <==
\label{sec:converse}
%\begin{thm}
%\label{thm:converse}
%If the degree-of-freedom pair $(d_1,d_2)$ is achievable, then $(d_1,d_2) \in \D$.
%\end{thm}
%\begin{IEEEproof}[Sketch of Converse]
%\end{IEEEproof}

%%\ashuNote{remove theorem statement and just state the sketch of converse}
%The full converse is omitted, for brevity, but here we give a sketch of the procedure for showing the converse part of Theorem~\ref{thm:mainResult}.
%We would like to show that if the degree-of-freedom pair $(d_1,d_2)$ is achievable, then $(d_1,d_2) \in \D$.
%%\evanNote{Finish this} 
%It is easy to see that if $(d_1,d_2)$ is achievable, then constraints (\ref{eq:d1Bound}) and (\ref{eq:d2Bound}) must be satisfied as these are the point-to-point bounds given in \cite{TsePoon05DOF_EM}. 
%It remains to show that the sum degree-of-freedom constrain (\ref{eq:dSumBound}) must hold for every achievable $(d_1,d_2)$. 
%Our process for showing (\ref{eq:dSumBound}) is twofold. %First, a genie expands each of the scattering intervals until the interference and signal-of-interest intervals are overlapping and identical. The genie also lengthens each of the arrays such that the any added interference due to the overlapping scattering intervals is compensated so that the net manipulation of the genie only enlarge $\D$. 
%
%First, a genie expands the scattering intervals $\IntT{22}$ and $\IntT{12}$, to $\IntTPrime{22} = \IntTPrime{12} = \IntT{22} \cup \IntT{12}$,  and also expands $\IntR{11}$ and $\IntR{12}$ to  $\IntRPrime{11} = \IntRPrime{12} = \IntR{11} \cup \IntR{12}$. The genie also lengthens the $T_2$ array to $\LenTwoTxPrime = \LenTwoTx +  \LenOneRx \frac{|\IntR{11} \setminus \IntR{12}|} {|\IntT{22} \cup \IntT{12}|}$ and the $R_1$ array to length $\LenOneRxPrime = \LenOneRx +  \LenTwoTx \frac{|\IntT{22} \setminus \IntT{12}|} {|\IntR{11} \cup \IntR{12}|},$
%which one can show ensures that any added interference due to the expansion of $\IntT{12}$ and $\IntR{12}$ is compensated by the larger arrays sizes so that the net manipulation of the genie can only enlarge $\D$. 
%
%%each of the scattering intervals until the interference and signal-of-interest intervals are overlapping and identical. The genie also lengthens each of the arrays such that the any added interference due to the overlapping scattering intervals is compensated so that the net manipulation of the genie only enlarge $\D$. 
%
%One can check that after above genie manipulation is performed, the maximum of the $T_2$ and $R_1$ signaling dimensions are equal to $\dSumMax$ in constraint (\ref{eq:dSumBound}), and
%since the scattering intervals are overlapped, the channel model becomes the Hilbert space equivalent of the well-studied MIMO $Z$-channel. The Hilbert space analog to the bounding techniques employed in \cite{{Ke12ZDoF,Jafar07MIMOInterferenceDoF}} that show the sum degrees of freedom of the MIMO $z$-channel is bound by $\max(M_2,N_1)$ can be leveraged to show (\ref{eq:dSumBound}) as desired. 
%
%%First, let a genie increase $\LenOneTx$ and $\LenTwoRx$, the aperture size of the $T_1$ and $R_2$ arrays, towards infinity, such that the sum degrees of freedom becomes limited only by the signaling dimensions available at $T_2$ and $R_1$. Clearly, this genie will only increase the sum degrees of freedom.  

==> cornerCaseTable_long.tex <==
\begin{table}[htdp]
\caption{default}
\begin{center}
\begin{tabular}{c|c}
Case & $d_2' = \min\{\dTwoMax, \dSumMax - \dOneMax\}$ \tabularnewline
\hline
\begin{tabular}{c}
$\scriptstyle \LenOneTx|\IntT{11}|  \geq  \LenOneRx|\IntR{11}|,$ \tabularnewline
$\scriptstyle \LenTwoTx|\IntT{12}|  \geq  \LenOneRx|\IntR{12}|,$ \tabularnewline
$\scriptstyle \LenTwoRx|\IntR{22}|  \geq  \LenTwoTx|\IntT{22}|$
\end{tabular} 
& 
$2\min\{\LenTwoTx |\IntT{22}|, \LenTwoTx|\IntT{22}\cup\IntT{12}| - \LenOneRx|\IntR{11}\cap\IntR{12}| \}$
\tabularnewline \hline
%
\begin{tabular}{c}
$\scriptstyle \LenOneTx|\IntT{11}|  \geq  \LenOneRx|\IntR{11}|,$ \tabularnewline
$\scriptstyle \LenTwoTx|\IntT{12}|  \geq  \LenOneRx|\IntR{12}|,$ \tabularnewline
$\scriptstyle \LenTwoRx|\IntR{22}|  <  \LenTwoTx|\IntT{22}|$
\end{tabular} 
& 
$2\min\{\LenTwoRx |\IntR{22}|, \LenTwoTx|\IntT{22}\cup\IntT{12}| - \LenOneRx|\IntR{11}\cap\IntR{12}| \}$
\tabularnewline \hline
%
\begin{tabular}{c}
$\scriptstyle \LenOneTx|\IntT{11}|  \geq  \LenOneRx|\IntR{11}|,$ \tabularnewline
$\scriptstyle \LenTwoTx|\IntT{12}|  <  \LenOneRx|\IntR{12}|,$ \tabularnewline
$\scriptstyle \LenTwoRx|\IntR{22}|  \geq  \LenTwoTx|\IntT{22}|$
\end{tabular} 
& 
$2\min\{\LenTwoTx|\IntT{22}|, \LenTwoTx|\IntT{22}\setminus\IntT{12}|+ \LenOneRx |\IntR{12}\setminus\IntR{11}|\}$
\tabularnewline \hline
%
\begin{tabular}{c}
$\scriptstyle \LenOneTx|\IntT{11}|  \geq  \LenOneRx|\IntR{11}|,$ \tabularnewline
$\scriptstyle \LenTwoTx|\IntT{12}|  <  \LenOneRx|\IntR{12}|,$ \tabularnewline
$\scriptstyle \LenTwoRx|\IntR{22}|  <  \LenTwoTx|\IntT{22}|$
\end{tabular} 
& 
$2\min\{\LenTwoRx|\IntR{22}|, \LenTwoTx|\IntT{22}\setminus\IntT{12}|+ \LenOneRx |\IntR{12}\setminus\IntR{11}|\}$
\tabularnewline \hline
%
\begin{tabular}{c}
$\scriptstyle \LenOneTx|\IntT{11}|  <  \LenOneRx|\IntR{11}|,$ \tabularnewline
$\scriptstyle \LenTwoTx|\IntT{12}|  \geq  \LenOneRx|\IntR{12}|,$ \tabularnewline
$\scriptstyle \LenTwoRx|\IntR{22}|  \geq  \LenTwoTx|\IntT{22}|$
\end{tabular} 
& 
$2\min\{\LenTwoTx|\IntT{22}|, \LenTwoTx|\IntT{22}\cup\IntT{12}| + \LenOneRx|\IntR{11}\setminus\IntR{12}| - \LenOneTx|\IntT{11}| \}$
\tabularnewline \hline
%
\begin{tabular}{c}
$\scriptstyle \LenOneTx|\IntT{11}|  <  \LenOneRx|\IntR{11}|,$ \tabularnewline
$\scriptstyle \LenTwoTx|\IntT{12}|  \geq  \LenOneRx|\IntR{12}|,$ \tabularnewline
$\scriptstyle \LenTwoRx|\IntR{22}|  <  \LenTwoTx|\IntT{22}|$
\end{tabular} 
& 
$2\min\{\LenTwoRx|\IntR{22}|, \LenTwoTx|\IntT{22}\cup\IntT{12}| + \LenOneRx|\IntR{11}\setminus\IntR{12}| - \LenOneTx|\IntT{11}| \}$
\tabularnewline \hline
%
\begin{tabular}{c}
$\scriptstyle \LenOneTx|\IntT{11}|  <  \LenOneRx|\IntR{11}|,$ \tabularnewline
$\scriptstyle \LenTwoTx|\IntT{12}|  <  \LenOneRx|\IntR{12}|,$ \tabularnewline
$\scriptstyle \LenTwoRx|\IntR{22}|  \geq  \LenTwoTx|\IntT{22}|$
\end{tabular} 
& 
$2\min\{\LenTwoTx|\IntT{22}|, \LenTwoTx|\IntT{22}\setminus\IntT{12}| + \LenOneRx|\IntR{11}\cup\IntR{12}| - \LenOneTx|\IntT{11}| \}$
\tabularnewline \hline
%
\begin{tabular}{c}
$\scriptstyle \LenOneTx|\IntT{11}|  <  \LenOneRx|\IntR{11}|,$ \tabularnewline
$\scriptstyle \LenTwoTx|\IntT{12}|  <  \LenOneRx|\IntR{12}|,$ \tabularnewline
$\scriptstyle \LenTwoRx|\IntR{22}|  <   \LenTwoTx|\IntT{22}|$
\end{tabular} 
& 
$2\min\{\LenTwoRx|\IntR{22}|, \LenTwoTx|\IntT{22}\setminus\IntT{12}| + \LenOneRx|\IntR{11}\cup\IntR{12}| - \LenOneTx|\IntT{11}| \}$
\tabularnewline \hline
%
\end{tabular}
\end{center}
\label{default}
\end{table}%

==> notation.tex <==
The function $1(\mathsf{cond})$ is an indicator function that evaluates to one if the condition, $\mathsf{cond}$, is true, and otherwise evaluates to zero. Lowercase bold symbols such as $\boldsymbol{x}$ denote vectors, upper-case bold symbols such as $\boldsymbol{H}$ denote matrices, and uppercase sans-serif symbols such as $\mathsf{H}$ denote operators on scalar-valued functions. 

\textcolor{red}{Seems like that this a few things could be introduced later - awkward to just have these separately in the intro.} \evanNote{Agreed. Will move it. }
